TC-DTW: Accelerating Multivariate Dynamic Time Warping Through Triangle Inequality and Point Clustering

Dynamic time warping (DTW) plays an important role in analytics on time series. Despite the large body of research on speeding up univariate DTW, the method for multivariate DTW has not been improved much in the last two decades. The most popular algorithm used today is still the one developed seventeen years ago. This paper presents a solution that, as far as we know, for the first time consistently outperforms the classic multivariate DTW algorithm across dataset sizes, series lengths, data dimensions, temporal window sizes, and machines. The new solution, named TC-DTW, introduces Triangle Inequality and Point Clustering into the algorithm design on lower bound calculations for multivariate DTW. In experiments on DTW-based nearest neighbor finding, the new solution avoids as much as 98% (60% average) DTW distance calculations and yields as much as 25X (7.5X average) speedups.

==> Makefile <==
SOURCES	= \
	main.tex

.PHONY: default all rebuild clean

default:
	pdflatex main

all:
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main
#	dvips -Ppdf -G0 -t letter -e 0 -o main.ps main.dvi
#	ps2pdf -dPDFSETTINGS=/prepress  main.ps

refs:
	bibtex main
clean:
	-rm -rf main.aux main.bbl main.blg main.dvi main.log main.pdf main.ps *~
sources:
	@echo  ${SOURCES}

